Do you really code? Designing and Evaluating Screening Questions for Online Surveys with Programmers

Recruiting professional programmers in sufficient numbers for research studies can be challenging because they often cannot spare the time, or due to their geographical distribution and potentially the cost involved. Online platforms such as Clickworker or Qualtrics do provide options to recruit participants with programming skill; however, misunderstandings and fraud can be an issue. This can result in participants without programming skill taking part in studies and surveys. If these participants are not detected, they can cause detrimental noise in the survey data. In this paper, we develop screener questions that are easy and quick to answer for people with programming skill but difficult to answer correctly for those without. In order to evaluate our questionnaire for efficacy and efficiency, we recruited several batches of participants with and without programming skill and tested the questions. In our batch 42% of Clickworkers stating that they have programming skill did not meet our criteria and we would recommend filtering these from studies. We also evaluated the questions in an adversarial setting. We conclude with a set of recommended questions which researchers can use to recruit participants with programming skill from online platforms.

==> tables_plots/iterations.tex <==
\begin{table}[h!]
\centering 
\footnotesize
\begin{adjustbox}{max width=\textwidth, max totalheight=\textheight} 
\begin{tabular}{lcc}
\toprule
\textbf{Iteration Name}&\textbf{Samples}&\textbf{n}  \\ 
\midrule
\multirow{2}{*}{\textbf{Developer}}&
Computer Science Students &17  
 \\ 
%&Clickworker with programming in profile & 50
& Professional Developers& 33 \\
%\midrule
\addlinespace[0.2cm]
\multirow{2}{*}{\textbf{Non-Developer}}&
Econ students& 50 \\
& Clickworker without programming experience& 50 \\ 
%\midrule
\addlinespace[0.2cm]
\textbf{Test group}&  
Clickworker with programming in profile& 52  \\
\newtext{\textbf{Attack scenario}}&   Clickworker without programming in profile& 47 \\

%\midrule
%\cellcolor{LightGray}
%Total & \\
\bottomrule
\end{tabular} 
\end{adjustbox} 
\caption{Iterations} 
\label{tab:questions_iterations} 
\end{table} 

==> tables_plots/iterations2.tex <==
\begin{table}[h!]
\centering 
\footnotesize
\begin{adjustbox}{max width=\textwidth, max totalheight=\textheight} 
\begin{tabular}{lp{3cm}cp{1.5cm}}
\toprule
\textbf{Iteration Name}&\textbf{Samples}&\textbf{n} & \textbf{Questions} \\ 
\midrule
\multirow{2}{*}{\textbf{Developer}}&
Computer Science Students &17  & Q1-Q16
 \\ 
%&Clickworker with programming in profile & 50
& Professional Developers& 33 & Q1-Q16\\
%\midrule
\addlinespace[0.2cm]
\multirow{2}{*}{\textbf{Non-Developer}}&
Econ students& 50 & 
Q1-Q16 \\
& Clickworker without programming experience& 50 &Q1-Q16\\ 
%\midrule
\addlinespace[0.2cm]
\textbf{Test group}&  
Clickworker with programming in profile& 52 &  Q1-Q16 \\
\newtext{\textbf{Attack scenario}}&   Clickworker without programming in profile& 47 & Q1-Q4, Q6, Q14-Q16\\

%\midrule
%\cellcolor{LightGray}
%Total & \\
\bottomrule
\end{tabular} 
\end{adjustbox} 
\caption{Iterations and Questions} 
\label{tab:questions_iterations} 
\end{table} 

==> tables_plots/participants_groups.tex <==
\begin{table}[h!]
\centering 
\footnotesize
\begin{adjustbox}{max width=\textwidth, max totalheight=\textheight} 
\begin{tabular}{llc}
\toprule
\textbf{Category}&\textbf{Sample} & \textbf{n} \\ 
\midrule
\multirow{2}{*}{\textbf{Developer}}&
Computer Science Students  & 
17 \\ 
%&Clickworker with programming in profile & 50
& Professional Developers &33\\
%\midrule
\addlinespace[0.2cm]
\multirow{2}{*}{\textbf{Non-Developer}}&
Econ students & 
50 \\
& Clickworker without programming experience &50\\ 
%\midrule
\addlinespace[0.2cm]
\textbf{Test group}&  
Clickworker with programming in profile &  52\\
\newtext{\textbf{Attack Scenario}} & Clickworker without programming experience & xx\\
\midrule
%\cellcolor{LightGray}
&Total & 202\\
\bottomrule
\end{tabular} 
\end{adjustbox} 
\caption{Groups and number of participants} 
\label{tab:groups} 
\end{table} 

==> tables_plots/table_demographics.tex <==
\begin{table*}[h] \centering
\scriptsize
\begin{adjustbox}{max width = \textwidth,  max totalheight = \textheight} 
\begin{tabular}{p{2.5cm}p{2.5cm}p{2.5cm}|p{2.5cm}p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule 
%&\multicolumn{2}{c|}{\textit{Developer (n = 50)}}&\multicolumn{2}{c|}{\textit{Non-Developer (n = 100) }}&\textit{Test group}\\
&\multicolumn{2}{c|}{\textit{Developer}}&\multicolumn{2}{c|}{\textit{Non-Developer}}&\textit{Test group}&\textit{Attack group}\\
&&&&&\\
&\textbf{CS Students}&\textbf{Professional}&\textbf{Econ Students}&\textbf{Clickworker}&\textbf{Clickworker}&\textbf{Clickworker}\\
%&\textbf{Students }(n = 17)&\textbf{Developers }(n = 33)&\textbf{No Experience }(n = 50)&\textbf{No Experience }(n = 50)&\textbf{Experience }(n = 52)\\
&\textbf{}&\textbf{Developers }&\textbf{}&\textbf{No Experience }&\textbf{Experience }&\textbf{Attack Scenario}\\
%\rowcolor{LightGray}\textbf{Sample Size} &n = 17&n = 33&n = 50&n = 50&n = 52\\ 
\midrule
\rowcolor{LightGray}\textbf{Gender}&female: 4, male: 13&female: 2, male: 31&female: 36, male: 13, prefer not to tell: 1&female: 20, male: 29, pref not to tell: 1&female: 10, male: 41, pref not to tell: 1&female: 18, male: 28, pref not to tell: 1\\ 
\textbf{Age}&min: 19, max: 30, mean: 21.82, md: 20, sd: 3.26 &min: 25, max: 55, mean: 36.45, md: 36, sd: 8.04 &min: 18, max: 28, mean: 22.66, md: 23, sd: 2.3&min: 19, max: 67, mean: 34.02, md: 31.5, sd:10.43&min: 18, max: 58, mean: 33.73, md: 31.5, sd: 9.81&min: 19, max: 54, mean: 32.15, md: 30, sd: 9.15\\ 
%\textbf{Main Occupation}&CS Student&Developers \& IT-professionals (see appendix for whole list)&Student (Economy, Biology, Physics):  48, Trainee:  2,  NA:  2&e.g Administrator,  Economist (see appendix for whole list)&e.g Graphic Designer,  Architect,  (see appendix for whole list)&e.g Student, Factory Technician (see appendix for whole list)\\ 
\rowcolor{LightGray}\textbf{Country of Residence}&Germany:  17&Germany: 31,  Austria:  2&Germany: 49,  NA: 1&Germany:    21,    UK: 8,    USA:    6,    Other: 15 (see appendix for whole list)&Germany: 22,  UK: 5,  Other: 25 (see appendix for whole list)&Germany: 16, Italy: 4, Spain: 4, USA: 4, Other: 19 (see appendix for whole list) \\ 
\textbf{General Development Experience [years]}&min: 2, max: 16, mean: 5.31,  md: 4.5, sd: 3.41, NA:  1 &min: 2,  max: 30,  mean: 13.09,  md: 15, sd: 7.31 &min: 0, max: 2, mean: 0.21,  md: 0, sd: 0.52 &min: 0,  max: 25,  mean: 1.63,  md: 0.25, sd: 4.1 &min: 0,  max: 30,  mean: 6.08,  md: 3, sd: 7.78, NA: 1&min: 0,  max: 26,  mean: 2.22,  md: 1, sd: 4.82\\ 



\bottomrule
\end{tabular}
\end{adjustbox}

\caption{Demographics of the Participants (n = 249)}
\textbf{Experience: } programming experience; \textbf{md: } median.
\label{tab: demographics} 

\end{table*} 

==> tables_plots/table_q_unsorted.tex <==
\begin{table} [hb]
\centering 
\begin{adjustbox}{max width=\textwidth, max totalheight=\textheight} \begin{tabular}{ccccc}
\toprule

\textbf{No}&\textbf{Question}&\textbf{Developers}&\textbf{Non-Developers}&\textbf{Test group}\\
\midrule
Q1&Unknown.Languages&98.00\%&91.00\%&96.15\%\\ 
Q2&Source.Usage&100.00\%&6.00\%&57.69\%\\ 
Q3&Compiler&100.00\%&33.00\%&78.84\%\\ 
Q4&Recursive&100.00\%&30.00\%&78.84\%\\ 
Q5&Algorithm&98.00\%&47.00\%&90.38\%\\ 
Q6&Boolean&100.00\%&25.00\%&78.84\%\\ 
Q7&Power.of.2&96.00\%&41.00\%&76.92\%\\ 
Q8&Bin.Conv&96.00\%&38.00\%&76.92\%\\ 
Q9&Bin.Even&90.00\%&34.00\%&61.53\%\\ 
Q10&Hexa.Num&70.00\%&6.00\%&57.69\%\\ 
Q11&Error.Overflow&94.00\%&21.00\%&67.30\%\\ 
Q12&Runtime&80.00\%&6.00\%&28.74\%\\ 
Q13&Error.OutOfBound&76.00\%&9.00\%&32.69\%\\ 
Q14&Sorting.Array&98.00\%&24.00\%&59.61\%\\ 
Q15&Function.Param&100.00\%&13.00\%&63.46\%\\ 
Q16&Backward.Loop&94.00\%&7.00\%&46.15\%\\ 
\bottomrule
\end{tabular} \end{adjustbox} \caption{...} \label{table:unsortedcomparison} \end{table} 

==> tables_plots/table_sim.tex <==
\begin{table*}[]\centering \footnotesize \begin{adjustbox}{max width=\textwidth, max totalheight=\textheight} 

\begin{tabular}{p{2.5cm}p{3cm}|ccccc|ccccc|cccccc}
\toprule
&&\multicolumn{5}{c}{\textbf{Number of Developer} (n = 50) }&\multicolumn{5}{c}{\textbf{Number of Non-Developer} (n = 100)} &\multicolumn{5}{c}{\textbf{Number of Test Group} (n = 52)} \\ 
Configuration&Questions &max&min&mean&md&sd&max&min&mean&md&sd&max&min&mean&md&sd\\
\midrule
2 out of 12 (2 correct)&Q2-Q9, Q11, Q14-Q16&     50&  42&   47.27&  47.0& 1.42 & 21&  4&  11.37&  11&  2.44&     38& 
     20&
     28.97&
     29.0&
     2.44\\
\rowcolor{LightGray}2 out of 5 (2 correct)&Q2, Q15, Q6, Q4, Q3&   50&
     50&
     50.0& 
     50.0& 
     0.0& 16&  2&  8.18&  8.00&  2.04&     39& 
     22& 
     30.11& 
     30.0& 
     2.15\\ 
5 out of 12 (3 correct)&Q2-Q9, Q11, Q14-Q16&   50& 
     49& 
     49.95& 
     50.0& 
     0.22& 29&  9&  18.04&  18&  2.48&     44& 
     32& 
     37.45& 
     37.0& 
     1.86\\ 



\bottomrule
\end{tabular} \end{adjustbox} \caption{Configuration and results of 3 example simulations.}
\small The table denotes how many participants would have correctly answered the randomly chosen questions in $10\,000$ simulations in each group. \\
md: median 
sd: standard deviation
\label{table:simulation} \end{table*} 
